Transaction Monitoring of Smart Contracts

Blockchains are modern distributed systems that provide decentralized financial capabilities with trustable guarantees. Smart contracts are programs written in specialized programming languages running on a blockchain and govern how tokens and cryptocurrency are sent and received. Smart contracts can invoke other contracts during the execution of transactions initiated by external users. Once deployed, smart contracts cannot be modified and their pitfalls can cause malfunctions and losses, for example by attacks from malicious users. Runtime verification is a very appealing technique to improve the reliability of smart contracts. One approach consists of specifying undesired executions (never claims) and detecting violations of the specification on the fly. This can be done by extending smart contracts with additional instructions corresponding to monitor specified properties, resulting in an onchain monitoring approach. In this paper, we study transaction monitoring that consists of detecting violations of complete transaction executions and not of individual operations within transactions. Our main contributions are to show that transaction monitoring is not possible in most blockchains and propose different execution mechanisms that would enable transaction monitoring.

==> Contracts/BadClient.tex <==
\begin{figure}[t!]
\begin{lstlisting}[language=Solidity,numbers=none,caption=Malicious client for a flash loan, label={flashLoan:badClient}]
  contract BadClient {
    Lender l;
    function borrowAndInvest() public {
      l.lend(100); 
      invest(100);
    }
  }
\end{lstlisting}
  \end{figure}

%%% Local Variables:
%%% TeX-master: "../article.tex"
%%% TeX-PDF-mode: t
%%% End:


==> Contracts/Client.tex <==
\begin{figure}[th!]
\vspace{-0.5em}  
\begin{lstlisting}[language=Solidity,numbers=none,caption=Possible client for a flash loan,label={flashLoan:client}]
  contract Client {
    Lender l1, l2;
    function borrowAndInvest() public {
      l1.lend(100);l2.lend(200);
      invest(300); 
      l1.transfer(100);l2.transfer(200);
    }
  }
\end{lstlisting}  \end{figure}

%%% Local Variables:
%%% TeX-master: "../article.tex"
%%% TeX-PDF-mode: t
%%% End:


==> Contracts/Flashloan.tex <==
\begin{figure}[t!]
\begin{lstlisting}[language=Solidity,numbers=none,caption=A Flash Loan implementation attempt,label={flashLoan:lender}]
  contract Lender {
    function lend(address payable dest, uint amount) public {
      require(amount <= this.balance);
      uint initial_balance = this.balance; 
      dest.transfer(amount); 
      assert(this.balance >= initial_balance); 
    }
  }
\end{lstlisting}
\end{figure}

%%% Local Variables:
%%% TeX-master: "../article.tex"
%%% TeX-PDF-mode: t
%%% End:


==> Contracts/Flashloan_monitor_fee.tex <==
\begin{figure}[t!]
\begin{lstlisting}[language=Solidity,numbers=none,caption=A correct Flash Loan implementation with transaction monitors]
  contract Lender {
    uint pending_to_receive monitor_storage; 
    function lend(address payable dest, uint amount) public {
      require(amount <= this.balance);
      dest.transfer(amount); 
    }
    function term() monitor {
      assert(pending_to_receive == 0); 
    }
    function lend_begin(uint amount) monitor {
      pending_to_receive += amount + amount / 100;
    }
    function transfer_begin() monitor {
      pending_to_receive -= msg.value;
    }

  }
\end{lstlisting}\label{flashLoan:lenderFeeWithTransactionMonitor}
\end{figure}

%%% Local Variables:
%%% TeX-master: "../article.tex"
%%% TeX-PDF-mode: t
%%% End:


==> Contracts/Flashloan_monitor_withdraw.tex <==
\begin{figure}[t!]
\begin{lstlisting}[language=Solidity,numbers=none,caption=A Flash Loan implementation with transaction monitors and a withdraw function for the owner]
  contract Lender {
    address public owner;
    uint initial_balance monitor_storage;
    uint withdrawn_by_owner monitor_storage;    

    function lend(address payable dest, uint amount) public {
      require(amount <= this.balance);
      dest.transfer(amount);
    }
    function withdraw(uint amount) public {
      require(amount <= this.balance); 
      require(msg.sender == owner); 
      owner.transfer(amount); 
    }
    function init() monitor {
      initial_balance = this.balance;
      withdrawn_by_owner = 0; 
    } 
    function term() monitor {
      assert(this.balance >= initial_balance - withdrawn_by_owner); 
    }
    function withdraw_begin(uint amount) monitor {
      withdrawn_by_owner += amount;
    }
  }
\end{lstlisting}\label{flashLoan:lenderWithTransactionMonitorAndOwnerWithdrawing}
\end{figure}

%%% Local Variables:
%%% TeX-master: "../article.tex"
%%% TeX-PDF-mode: t
%%% End:


==> figures/latex/programs.tex <==
\newcommand{\RefFigListClass}{\ref{fig:programs}(a)\xspace}
\newcommand{\RefFigMGC}      {\ref{fig:programs}(b)\xspace}
\newcommand{\RefFigSearch}   {\ref{fig:programs}(c)\xspace}
\newcommand{\RefFigLocate}   {\ref{fig:programs}(d)\xspace}
\newcommand{\RefFigAdd}      {\ref{fig:programs}(e)\xspace}
\newcommand{\RefFigRemove}   {\ref{fig:programs}(f)\xspace}

\newcommand{\RefFigListClassGhost}{\ref{fig:programs:ghost}(a)\xspace}
\newcommand{\RefFigLocateGhost}		{\ref{fig:programs:ghost}(b)\xspace}
\newcommand{\RefFigAddGhost}			{\ref{fig:programs:ghost}(c)\xspace}
\newcommand{\RefFigRemoveGhost}		{\ref{fig:programs:ghost}(d)\xspace}

\newcommand{\FigLabel}[1]{\multicolumn{1}{c}{#1}}
\newcommand{\FigLabelWide}[1]{\multicolumn{3}{c}{#1}}

%
% Figures for data structure
%
\newcommand{\ListDataStructuresBody}{
  \begin{array}{l>{\hspace{0.25em}}l<{\hspace{0.25em}}l}
	  \class & \List & \{ \Node \: \tList; \; \} \\
	  \class & \Node & \{
			\Value \: \val; \;
			\Node \: \tNext; \;
			\Lock \: \lock; \; \}
  \end{array}
}



%
% Figures for most generate cliente "decide"
%
\newcommand{\ListMGCBody}{
  \begin{algorithmic}[1]
	\Procedure{MGC}{}
	  \While {$\true$}
	  \State $e := \NondetChooseElem$
	  \State $\Nondet$
	  \State $\left[ \begin{array}{l}
		\Call \search(e) \\
		\ProgOr \\
		\Call \insertProg(e) \\
		\ProgOr \\
		\Call \remove(e)
	  \end{array} \right]$
	  \EndWhile
	\EndProcedure
  \end{algorithmic}
}



%
% Figure for "search" 
%

\newcommand{\ListSearchBody}{
  \begin{algorithmic}[1]
	\Procedure{Search}{$\Value \: e$}
	\State $\prev, \curr := \locate(e)$
    \If {$\curr.\val = e$}
    \State $\result := \true$
    \Else
    \State $\result := \false$
    \EndIf
    \State $\curr.\unlock()$
    \State $\prev.\unlock()$
    \State \tbf{return} $\result$
	\EndProcedure
  \end{algorithmic}
}



%
% Figure for "locate"
%
\newcommand{\ListLocateBody}{
  \begin{algorithmic}[1]
	\Procedure{Locate}{$\Value \: e$}
	  \State $\prev := \Head$
	  \State $\prev.\lock()$
	  \State $\curr := \prev.\tNext$
	  \State $\curr.lock()$
	  \While {$\curr.\val < e$}
		\State $\prev.\unlock()$
		\State $\prev := \curr$
		\State $\curr := \curr.\tNext$
		\State $\curr.\lock()$
	  \EndWhile
	  \State \tbf{return} $(\prev, \curr)$
	\EndProcedure
  \end{algorithmic}
}



%
% Figure for "add"
%
\newcommand{\ListAddBody}{
  \begin{algorithmic}[1]
	\Procedure{Insert}{$\Value \: e$}
	  \State $\prev, \curr := \locate(e)$
	  \If {$\curr.\val \neq e$}
		\State $\aux := \New \Node(e)$
		\State $\aux.\tNext := \curr$
		\State $\prev.\tNext := \aux$
		\State $\result := \true$
	  \Else
		\State $\result := \false$
	  \EndIf
	  \State $\prev.\unlock()$
	  \State $\curr.\unlock()$
	  \State \tbf{return} $\result$
	\EndProcedure
  \end{algorithmic}
}



%
% Figure for "remove"
%
\newcommand{\ListRemoveBody}{
    \begin{algorithmic}[1]
	  \Procedure{Remove}{$\Value \: e$}
		\State $\prev, \curr := \locate(e)$
		\If {$\curr.\val = e$}
		  \State $\aux := \curr.\tNext$
		  \State $\prev.\tNext := \aux$
		  \State $\result := \true$
		\Else
		  \State $\result := \false$
		\EndIf
		\State $\prev.\unlock()$
		\State $\curr.\unlock()$
		\State \tbf{return} $\result$
	  \EndProcedure
	\end{algorithmic}
}




%
% Figures for data structure
%
\newcommand{\DataStructuresGhostBody}{
	\begin{tabular}{cc}
		\renewcommand{\arraystretch}{0.4}
		$\begin{array}{l}
			\class \: \List \: \{ \\
			\mhs \Node \: \tList ;\\
			\hs{0.2} \fbox{ \begin{array}{l}
				\rgn \: r; \\
			\end{array}}\\
		\}
		\end{array}$ & \hs{2} $\begin{array}{l}
			\class \: \Node \: \{ \\
			\mhs \Value \: \val ;\\
			\mhs \Node \: \tNext ;\\
			\mhs \Lock \: \lock ;\\
		\}
	\end{array}$
	\end{tabular}
}

\newcommand{\DataStructuresGhostFig}{
\begin{minipage}[c]{6.5cm}
	\DataStructuresGhostBody
\label{fig:conclists:ghost}
\end{minipage}
}


%
% Figure for "locate" extended with ghost fields
%

\newcommand{\ListLocateGhostBody}{
  \begin{algorithmic}[1]
	\Procedure{Locate}{$\Value \: e$}
	  \State $\prev := \Head$
	  \State $\prev.\lock()$
	  \State $\curr := \prev.\tNext$
	  \State $\curr.lock()$
	  \While {$\curr.\val < e$}
		\State $\prev.\unlock()$
		\State $\prev := \curr$
		\State $\curr := \curr.\tNext$
		\State $\curr.\lock()$
	  \EndWhile
	  \State \tbf{return} $(\prev, \curr)$
	\EndProcedure
  \end{algorithmic}
}


%
% Figure for "add" extended with ghost fields
%
\newcommand{\ListAddGhostBody}{
  \begin{algorithmic}[1]
	\Procedure{Insert}{$\Value \: e$}
	  \State $\prev, \curr := \locate(e)$
	  \If {$\curr.\val \neq e$}
		\State $\aux := \New \Node(e)$
		\State $\aux.\tNext := \curr$
		\State $\prev.\tNext := \aux$
		\Statex $\hs{0.7}\fbox{
		  \begin{array}{l}
			l.r := l.r \cup \sreg{\aux} \\
		  \end{array}}$
		\State $\result := \true$
	  \Else
		\State $\result := \false$
	  \EndIf
	  \State $\prev.\unlock()$
	  \State $\curr.\unlock()$
	  \State \tbf{return} $\result$
	\EndProcedure
  \end{algorithmic}
}



%
% Figure for "remove" extended with ghost fields
%
\newcommand{\ListRemoveGhostBody}{
  \begin{algorithmic}[1]
	\Procedure{Remove}{$\Value \: e$}
	  \State $\prev, \curr := \locate(e)$
	  \If {$\curr.\val = e$}
		\State $\aux := \curr.\tNext$
		\State $\prev.\tNext := \aux$
		\Statex $\hs{0.7}\fbox{
		  \begin{array}{l}
			l.r := l.r - \sreg{\curr} \\
		  \end{array}}$
		\State $\result := \true$
	  \Else
		\State $\result := \false$
	  \EndIf
	  \State $\prev.\unlock()$
	  \State $\curr.\unlock()$
	  \State \tbf{return} $\result$
	\EndProcedure
  \end{algorithmic}
}


%
% Figure for data structure for proving no overtake
%
\newcommand{\DataStructuresGhostTicketBody}{
	\begin{tabular}{c>{\hspace{1cm}}c}
		\renewcommand{\arraystretch}{0.4}
		$\begin{array}{l}
			\class \: \List \: \{ \\
			\mhs \Node \: \tList ;\\
			\hs{0.2} \fbox{ \begin{array}{l}
				\rgn \: r; \\
			\end{array}} \\
		\}
		\end{array}$ & 
		$\begin{array}{l}
			\class \: \Node \: \{ \\
			\mhs \Value \: \val ;\\
			\mhs \Node \: \tNext ;\\
			\mhs \Lock \: \lock ;\\
		\}
	\end{array}$
	\end{tabular}
}

\newcommand{\DataStructuresGhostTicketFig}{
\begin{minipage}[c]{5cm}
	\DataStructuresGhostTicketBody
\label{fig:struct-cl-ticket}
\end{minipage}
}



%
% Figure for "locate" extended with ghost fields for proving no overtake
%

\newcommand{\ListLocateGhostTicketBody}{
  \begin{algorithmic}[1]
	\Procedure{Locate}{$\Value \: e$}
	  \State $\prev := \Head$
	  \State $\prev.\lock()$
	  \Statex $\hs{0.7}\fbox{
		\begin{array}{l}
		  \myTicket := \ticket \\
		  \ticket := \ticket + 1 \\
		\end{array}}$
	  \State $\curr := \prev.\tNext$
	  \State $\curr.lock()$
	  \While {$\curr.\val < e$}
		\State $\prev.\unlock()$
		\State $\prev := \curr$
		\State $\curr := \curr.\tNext$
		\State $\curr.\lock()$
	  \EndWhile
	  \State \tbf{return} $(\prev, \curr)$
	\EndProcedure
  \end{algorithmic}
}




\newcommand{\RefFigSkiplistClass}{\ref{fig:programs}(a)\xspace}
\newcommand{\RefFigInsert}{\ref{fig:programs}(b)\xspace}

%
% Figures for data structure
%
\newcommand{\SkiplistDataStructuresBody}{
	\begin{array}{l>{\hspace{0.25em}}l>{\hspace{0.25em}}llll}
		\class & \SkipList & \{ &
			\NodeP & \head; \; \\
			&&& \NodeP & \tail; \\
			&&& \Tint & \maxLevel; \\
			&&& \TSet{\Addr} & @\reg; & \} \\
		\class & \Node & \{ &
			\Value & \val;		\\
			&&& \Key & \key;	\\
			&&& \TArray \langle \NodeP \rangle & \fNext; \\
			&&& \Tint & @\level; & \}
%			&&& \TArray \langle \NodeP \rangle \: \lock; & \}
  \end{array}
}


\newcommand{\SkiplistInsertBody}{
%  \framebox[\textwidth]{
	\begin{algorithmic}[1]
	\Statex
	\Procedure{Insert}{$\SkipList \: sl$, $\Value \: \newval$}
	\MState {$\Tvector\tuple{\NodeP} \upd[0..K-1]$}
			{$\mrgn \: m_r := \emptyset$}{8}{0}
	\State $lvl := \randomLevel(K)$
	\State $\NodeP \pred := sl.\head$
	\MState {$\pred.\locks[K-1].\lock()$}
			{$m_r := m_r \cup \{ (\pred, K-1) \}$}{8}{0}
	\State $\NodeP \curr := \pred.\fNext[K-1]$
	\MState {$\curr.\locks[K-1].\lock()$}
			{$m_r := m_r \cup \{ (\curr, K-1) \}$}{8}{0}
	\For {$i:=K-1$ downto $0$}
		\If {$i < K -1$}
			\MState {$\pred.\locks[i].\lock()$}
					{$m_r := m_r \cup \{ (\pred, i) \}$}{8}{2}
			\If {$i \geq lvl$}
				\MState {$\curr.\locks[i+1].\unlock()$}
						{$m_r := m_r - \{ (\curr, i+1) \}$}{8}{3}
				\MState {$\pred.\locks[i+1].\unlock()$}
						{$m_r := m_r - \{ (\pred, i+1) \}$}{8}{3}
			\EndIf
			\State $\curr := \pred.\fNext[i]$
			\MState {$\curr.\locks[i].\lock()$}
					{$m_r := m_r \cup \{ (\curr, i) \}$}{8}{2}
		\EndIf
		\While {$\curr.\val < \newval$}
			\MState {$\pred.\locks[i].\unlock()$}
					{$m_r := m_r - \{ (\pred, i) \}$}{8}{2}
			\State $\pred := \curr$
			\State $\curr := \pred.\fNext[i]$
			\MState {$\curr.\locks[i].\lock()$}
					{$m_r := m_r \cup \{ (\curr, i) \}$}{8}{2}
		\EndWhile
		\State $\upd[i] := \pred$
	\EndFor
	\State $\bool \: \valueWasIn := (\curr.\val = \newval)$

	\If {$\valueWasIn$}
		\For {$i := 0$ to $lvl$}
			\MState {$\upd[i].\fNext[i].\locks[i].\unlock()$}
					{$m_r := m_r - \{ (\upd[i].\fNext[i], i)\}$}
						{8}{2}
			\MState {$\upd[i].\locks[i].\unlock()$}
					{$m_r := m_r - \{ (\upd[i], i) \}$}{8}{2}
		\EndFor
	\Else
		\State $x:=\CreateNode(lvl, \newval)$
		\For {$i:=0$ to $lvl$}
			\State $x.\fNext[i] := \upd[i].\fNext[i]$
			\MState {$\upd[i].\fNext[i] := x$}
					{$sl.r := sl.r \cup \{ (x, i) \}$}{8}{2}
			\MState {$x.\fNext[i].\locks[i].\unlock()$}
					{$m_r := m_r - \{ (x.\fNext[i], i) \}$}
						{8}{2}
			\MState {$\upd[i].\locks[i].\unlock()$}
					{$m_r := m_r - \{ (\upd[i], i) \}$}{8}{2}
		\EndFor
	\EndIf
	\State $\tbf{return } \lnot \valueWasIn$
	\EndProcedure
	\end{algorithmic}
%      }
}




==> figures/latex/theories.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TLLpL Signature
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TLLpLSignature}{
\centering
\begin{tabular}{r>{\vspace{-.5\baselineskip}}p{10.5cm}}
\hline
\textbf{Signature:} & \sigCells \\
\textbf{Sorts:} & \sCell, \sElem, \sAddr, \sThId \\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			\fError & : & \sCell \\
			\fMkcell & : & \sElem \times \sAddr \times \sThId \to \sCell \\
			\_.\fData & : & \sCell \to \sElem \\
			\_.\fNext & : & \sCell \to \sAddr \\
			\_.\fLockID & : & \sCell \to \sThId \\
			\_.\fLock & : & \sCell \to \sThId \to \sCell \\
			\_.\fUnlock & : & \sCell \to \sCell \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigMemory \\
\textbf{Sorts:} & \sMem, \sAddr, \sCell\\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			\fNull & : & \sAddr \\
			\_[\_] & : & \sMem \times \sAddr \to \sCell \\
			\fUpd & : & \sMem \times \sAddr \times \sCell \to \sMem \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigReach \\
\textbf{Sorts:} & \sMem, \sAddr, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			\fEpsilon & : & \sPath \\
			\lbrack \_ \rbrack & : & \sAddr \to \sPath \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{1.6cm}cl}
			\pAppend & : & \sPath \times \sPath \times \sPath \\
			\pReach & : & \sMem \times \sAddr \times \sAddr \times \sPath \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigSets \\
\textbf{Sorts:} & \sAddr, \sSet \\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			$\emptyset$ & : & \sSet \\
			\{ \_ \} & : & \sAddr \to \sSet \\
			$\cup$, $\cap$, $\setminus$ & : & \sSet \times \sSet \to \sSet
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{1.6cm}cl}
			$\in$ & : & \sAddr \times \sSet \\
			$\subseteq$ & : & \sSet \times \sSet
			\end{array} \\
\hline
\textbf{Signature:} & \sigSetsT \\
\textbf{Sorts:} & \sThId, \sSetT \\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			\stEmpty & : & \sSetT \\
			\stSingle{\_} & : & \sThId \to \sSetT \\
			\stCup, \stCap, \stSubst & : & \sSetT \times \sSetT \to \sSetT
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{1.6cm}cl}
			\stIn & : & \sThId \times \sSetT \\
			\stSubset & : & \sSetT \times \sSetT
			\end{array} \\
\hline
\textbf{Signature:} & \sigBridge \\
\textbf{Sorts:} & \sMem, \sAddr, \sSet, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{1.6cm}cl}
			\fPathToSet & : & \sPath \to \sSet \\
			\fAddrToSet & : & \sMem \times \sAddr \to \sSet \\
			\fGetp & : & \sMem \times \sAddr \times \sAddr \to \sPath \\
			\fFirstLocked & : & \sMem \times \sPath \to \sAddr
			\end{array} \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TLLpL Interpretations
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TLLpLInterpretations}{
\centering
\begin{tabular}{r>{\vspace{-.5\baselineskip}}p{10.5cm}}
\hline
\textbf{signature:} & \sigCells \\
\textbf{interpretation:} &
		\begin{compactitem}
		\item $\fMkcell (e, a, k) =
			\langle e, a, k \rangle$
		\item $\langle e, a, t \rangle.\inter{\fData}{\Ai} = e$
		\item $\langle e, a, t \rangle.\inter{\fNext}{\Ai} = a$
		\item $\langle e, a, t \rangle.\inter{\fLockID}{\Ai} = t$
		\item $\langle e, a, t \rangle.\inter{\fLock}{\Ai}(t') =
			\langle e, a, t' \rangle$
		\item $\langle e, a, t \rangle.\inter{\fUnlock}{\Ai} =
			\langle e, a, \oslash \rangle$
		\item $\inter{\fError}{\Ai}.\inter{\fNext}{\Ai} =
			\inter{\fNull}{\Ai}$
		\end{compactitem} \\
		& for each
			$e \in \Ais{\sElem}$,
			$a \in \Ais{\sAddr}$,
			$k \in \Ais{\sThId}$
			and $t, t' \in \Ais{\sThId}$ \\
\hline
\textbf{Signature:} & \sigMemory \\
\textbf{Interpretation:} &
		\begin{compactitem}
		\item $m\inter{[a]}{\Ai} = m(a)$
		\item $\inter{\fUpd}{\Ai}(m,a,c) = m_{a \mapsto c}$
		\item $\inter{m}{\Ai}(\inter{\fNull}{\Ai}) = \inter{\fError}{\Ai}$
		\end{compactitem} \\
		& for each
			$m \in \Ais{\sMem}$,
			$a \in \Ais{\sAddr}$ and
			$c \in \Ais{\sCell}$ \\
\hline
\textbf{Signature:} & \sigReach \\
\textbf{Interpretation:} &
		\begin{compactitem}
		\item $\inter{\fEpsilon}{\Ai}$ is the empty sequence
		\item $\inter{[i]}{\Ai}$ is the sequence containing $i \in 
			\Ais{\sAddr}$ as the only element
		\item $\left(\left[i_1,\ldots, i_n\right], \left[j_1, \ldots, 
			j_m\right], \left[i_1,\ldots, i_n, j_1,
				\ldots, j_m\right]
			\right) \in \inter{\pAppend}{\Ai}$ iff

			\mhs $i_k$ and $j_l$ are all distinct
		\item $\left(m, i, j, p\right) \in \inter{\pReach}{\Ai}$ iff
			\begin{compactitem}
				\item $i=j$ and $p = \fEpsilon$, or
				\item there exist addresses $i_1, \ldots, i_n \in
						\Ais{\sAddr}$ such that:
			\end{compactitem}
		\end{compactitem} \\
		& \hs{1.5} $\begin{array}{l>{\hspace{1em}}l}
			\trm{(a) } p = [i_1, \ldots, i_n] &
			\trm{(c) } m(i_r).\inter{\fNext}{\Ai} = i_{r+1}$,
				for $1 \leq r < n \\
			\trm{(b) } i_1 = i &
			\trm{(d) } m(i_n).\inter{\fNext}{\Ai} = j
		\end{array}$ \\
\hline
\textbf{Signature:} & \sigSets \\
\textbf{Interpretation:} &
		\begin{compactitem}
		\item The symbols $\emptyset$, $\{ \_ \}$, $\cup$, $\cap$,
				$\setminus$, $\in$ and $\subseteq$ are interpreted according
				to their standard interpretation over sets of addresses.
		\end{compactitem}\\
\hline
\textbf{Signature:} & \sigSetsT \\
\textbf{Interpretation:} &
		\begin{compactitem}
		\item The symbols $\stEmpty$, $\stSingle{\_}$, $\stCup$, $\stCap$,
				$\stSubst$, $\stIn$ and $\stSubset$ are interpreted according
				to their standard interpretation over sets of thread
				identifiers.
		\end{compactitem}\\
\hline
\textbf{Signature:} & \sigBridge \\
\textbf{Interpretation:} &
		\begin{compactitem}
		\item $\inter{\fAddrToSet}{\Ai}(m, i) = \big\{ j \in \Ais{\sAddr} 
			\:|\: \exists p \in \Ais{\sPath}$
				s.t. $(m,i,j,p) \in \pReach \big\}$

		\item $\inter{\fPathToSet}{\Ai}(p) = \{ i_1, \ldots, i_n\}$ for $p = 
			[i_1, \ldots, i_n] \in \Ais{\sPath}$

		\item $\inter{\fGetp}{\Ai}(m,i,j) =
			\begin{cases}
				p & \text{if } (m,i,j,p)
					\in \inter{\pReach}{\Ai} \\
				\fEpsilon & \text{otherwise}
			\end{cases}$
		\end{compactitem} \\
		
		& \hs{1} for each $m \in \Ais{\sMem}$,
		$p \in \Ais{\sPath}$ and $i,j \in \Ais{\sAddr}$ \\

		& \begin{compactitem}
		\item $\inter{\fFirstLocked}{\Ai}\left(m,[a_1, \ldots, 
			a_n]\right) =
			\left\{
			\begin{array}{ll}
			a_k &
			\trm{if there is } 1 \leq k \leq n \trm{ such that } \\
			& \trm{for all } 1 \leq j < k,
				m[a_j].\fLockID = \oslash \\
			& \trm{and } m[a_k].\fLockID \neq \oslash \\
			\fNull & \trm{otherwise }
			\end{array}
			\right.$
		\end{compactitem} \\
		& \hs{1} for each $m \in \Ais{\sMem}$ and
			$a_1, \ldots a_n \in \Ais{\sAddr}$ \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TLLpL PATH Auxiliary functions
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ListTPathFig}{
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{|c|}
\hline
$\fApp : \sSeq \times \sSeq \to \sSeq$ \\
\hline
$\fApp (\fNil, l) = l$ \\
$\fApp(\fCons(a,l), l') = \fCons(a, \fApp(l, l'))$ \\
\hline
\hline
$\fSeqToSet : \sSeq \to \sSet$ \\
\hline
$\fSeqToSet (\fNil) = \emptyset$ \\
$\fSeqToSet (\fCons(a,l)) = \{ a \} \cup \fSeqToSet(l)$ \\
\hline
\hline
$\fIsPath : \sSeq$ \\
\hline
$\fIsPath(\fNil)$ \\
$\fIsPath(\fCons(a, \fNil))$ \\
$\{a\} \nsubseteq \fSeqToSet(l) \land \fIsPath(l) \Impl
	\fIsPath(\fCons(a,l))$ \\
\hline
\hline
$\fLast : \sSeq \to \sAddr$ \\
\hline
$\fLast(\fCons(a, \fNil)) = a$ \\
$l \neq \fNil \Impl \fLast(\fCons(a, l)) = \fLast(l)$ \\
\hline
\hline
$\pIsReach : \sMem \times \sAddr \times \sAddr$ \\
\hline
$\pIsReach(m, a, a)$ \\
$m[a].\fNext = a' \land \pIsReach(m, a', b) \Impl \pIsReach(m, a, b)$ \\
\hline
\hline
$\pIsReachP : \sMem \times \sAddr \times \sAddr \times \sSeq$ \\
\hline
$\pIsReachP(m, a, a, \fNil)$ \\
$m[a].\fNext = a' \land \pIsReachP(m, a', b, p) \Impl
	\pIsReachP(m, a, b, \fCons(a, p))$ \\
\hline
\hline
$\fFirstMarked : \sMem \times \sSeq \times \sAddr$ \\
\hline
$\fFirstMarked (m, \fNil, \fNull)$ \\
	\Impl
	\fFirstMarked(m, p, j)$ \\
	\land
	\fFirstMarked(m, q, i) \Impl \fFirstMarked(m, p, i)$ \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TLLpL Auxiliary Functions
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ListAuxiliaryFunctions}{
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{|c|}
\hline
$\List : \sMem \times \sAddr \times \sSet$ \\
\hline
$\begin{array}{lcl}
	\List(h,a,r) & \Iff & \fNull \in \fAddrToSet(h, a)
		\land r = \fPathToSet(\fGetp(h, a, \fNull)) \\
\end{array}$\\
\hline
\hline
$\fa : \sMem \times \sAddr \to \sPath$ \\
\hline
$\fa(h,n) = \begin{cases}
		\fEpsilon & \trm{if } n = \fNull \\
		\fGetp(h, h[n].\fNext, \fNull) & \trm{if } n \neq \fNull \\
		\end{cases}$ \\
\hline
%
% Begin: Function removed to reduce space
%
\hline
$\fb : \sMem \times \sAddr \times \sAddr \times \sPath$ \\
\hline
$\begin{array}{lclll}
\fb(h, n, m, p) & \Iff & (n = \fNull \land p = \fEpsilon) \quad \lor \\
		& & \big(n \neq \fNull \land \pReach(h,n,m,\tilde{p})
			& \land & m=\fNull	\Impl \pAppend(p, \fNull, \tilde{p}) \\
		& & & \land & m\neq \fNull \Impl \pAppend(p,[m],\tilde{p}) \big)
\end{array}$ \\
\hline
%
% End: Function removed to reduce space
%
\hline
$\LastMarked : \sMem \times \sPath \to \sAddr$ \\
\hline
$\LastMarked(m, p) = \fFirstLocked(m, \fRev(p))$ \\
\hline
\hline
$\NoMarks : \sMem \times \sPath$ \\
\hline
$\NoMarks(m,p) \Iff \fFirstLocked(m,p) = \fNull$ \\
\hline
\hline
$\SomeMark : \sMem \times \sPath$ \\
\hline
$\SomeMark(m,p) \Iff \fFirstLocked(m,p) \neq \fNull$ \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSLK Signature - Table One
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TSLKSignatureOne}{
\centering
\begin{tabular}{r>{\vspace{-.5\baselineskip}}p{9cm}}
\hline
\textbf{Signature:} & \sigLevelK \\
\textbf{Sorts:} & \sLevelK \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			0,1, \ldots, \K-1 & : & \sLevelK \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			$<$  & : & \sLevelK \times \sLevelK \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigOrd \\
\textbf{Sorts:} & \sOrd \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fZero, \fInfty & : & \sOrd \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pOrd & : & \sOrd \times \sOrd \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigCells \\
\textbf{Sorts:} & \sCell, \sElem, \sOrd, \sLevelK, \sAddr \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fError & : & \sCell \\
			\fMkcell & : & \sElem \times \sOrd \times \sAddr^{\K}
							\to \sCell \\
			\_.\fData & : & \sCell \to \sElem \\
			\_.\fKey & : & \sCell \to \sOrd \\
			\_.\fNext \lbrack \_ \rbrack & : & \sCell \times \sLevelK
							\to \sAddr \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigMemory \\
\textbf{Sorts:} & \sMem, \sAddr, \sCell \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fNull & : & \sAddr \\
			\fRd & : & \sMem \times \sAddr \to \sCell \\
			\fUpd & : & \sMem \times \sAddr \times \sCell \to \sMem \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigReach \\
\textbf{Sorts:} & \sMem, \sAddr, \sLevelK, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fEpsilon & : & \sPath \\
			\lbrack \_ \rbrack & : & \sAddr \to \sPath \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pAppend & : & \sPath \times \sPath \times \sPath \\
			\pReachK & : & \sMem \times \sAddr \times \sAddr
							\times \sLevelK \times \sPath \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigSets \\
\textbf{Sorts:} & \sAddr, \sSet \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			$\emptyset$ & : & \sSet \\
			$\{ \_ \}$ & : & \sAddr \to \sSet \\
			$\cup$, $\cap$, $\setminus$ & : & \sSet \times \sSet
								\to \sSet \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			$\in$ & : & \sAddr \times \sSet \\
			$\subseteq$ & : & \sSet \times \sSet \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigBridge \\
\textbf{Sorts:} & \sMem, \sAddr, \sLevelK, \sSet, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fPathToSet & : & \sPath \to \sSet \\
			\fAddrToSetK & : & \sMem \times \sAddr \times \sLevelK
							\to \sSet \\
			\fGetpK & : & \sMem \times \sAddr \times \sAddr
							\times \sLevelK \to \sPath \\
			%\fThreadSubset & : & \sMem \times \sAddr \times \sAddr
							%\times \sLevelK \to \sSetT
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pOrdList & : & \sMem \times \sPath \\
			\end{array} \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSLK Signature - Table Two
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TSLKSignatureTwo}{
\centering
\begin{tabular}{r>{\vspace{-.5\baselineskip}}p{9cm}}
\hline
\textbf{Signature:} & \sigSetsT \\
\textbf{Sorts:} & \sThId, \sSetT \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\stEmpty & : & \sSetT \\
			\stSingle{\_} & : & \sThId \to \sSetT \\
			\stCup, \stCap, \stSubst & : & \sSetT \times \sSetT
								\to \sSetT \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\stIn & : & \sThId \times \sSetT \\
			\stSubset & : & \sSetT \times \sSetT \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigMrgn \\
\textbf{Sorts:} & \sMrgn, \sAddr, \sLevelK \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\mrgnEmpty & : & \sMrgn \\
			\mrgnSingle{\_, \_} & : & \sAddr \times \sLevelK \to \sMrgn \\
			\mrgnCup, \mrgnCap, \mrgnMinus & : & \sMrgn \times \sMrgn
							\to \sMrgn \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\mrgnIn & : & \sAddr \times \sLevelK \times \sMrgn \\
			\mrgnSubset & : & \sMrgn \times \sMrgn \\
			\mrgnDisj & : & \sMrgn \times \sMrgn \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigAArray \\
\textbf{Sorts:} & \sAArray, \sThId, \sAddr \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\aarrRd{\_}{\_} & : & \sAArray \times \sThId \to \sAddr \\
			\aarrUpd{\_}{\_}{\_} & : &
					\sAArray \times \sThId \times \sAddr \to \sAArray \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigLArray \\
\textbf{Sorts:} & \sLArray, \sThId, \sLevelK \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\larrRd{\_}{\_} & : & \sLArray \times \sThId \to \sLevelK \\
			\larrUpd{\_}{\_}{\_} & : &
					\sLArray \times \sThId \times \sLevelK \to \sLArray \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigBridge \\
\textbf{Sorts:} & \sMem, \sAddr, \sLevelK, \sSet, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fPathToSet & : & \sPath \to \sSet \\
			\fAddrToSetK & : & \sMem \times \sAddr \times \sLevelK
							\to \sSet \\
			\fGetpK & : & \sMem \times \sAddr \times \sAddr
							\times \sLevelK \to \sPath \\
			\fFirstLockedK & : & \sMem \times \sPath \times \sLevelK
							\to \sAddr \\
			%\fThreadSubset & : & \sMem \times \sAddr \times \sAddr
							%\times \sLevelK \to \sSetT
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pOrdList & : & \sMem \times \sPath \\
			\end{array} \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSLK Interpretations
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TSLKInterpretations}{
\centering
\begin{tabular}{p{11cm}}
\hline \\
\textbf{Signature:} $\sigCells$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
    \begin{compactitem}
		\item $\inter{\fMkcell}{\Ai} (e, k, \vect{a}) =
			\langle e, k, \vect{a} \rangle$
		\item $\inter{\fError}{\Ai}.\inter{\fNext}{\Ai} =
			\inter{\fNull}{\Ai}$
		\item $\langle e, k, \vect{a} \rangle
				.\inter{\fData}{\Ai} = e$
		\item $\langle e, k, \vect{a} \rangle
				.\inter{\fKey}{\Ai} = k$
		\item $\langle e, k, \vect{a} \rangle
				.\inter{\fNext}{\Ai}[j] = a_j$
		\end{compactitem} \\
    for each
			$e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$\vect{a} \in \Ais{\sAddr}^{\K}$ and
			$j \in \Ais{\sLevelK}$ \\
  \end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigMemory$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
		\begin{compactitem}
		\item $\inter{\fRd}{\Ai}(m,a) = m(a)$
		\item $\inter{\fUpd}{\Ai}(m,a,c) = m_{a \mapsto c}$
		\item $\inter{m}{\Ai}(\inter{\fNull}{\Ai}) = \inter{\fError}{\Ai}$
		\end{compactitem} \\
    for each
      $m \in \Ais{\sMem}$,
			$a \in \Ais{\sAddr}$
      and $c \in \Ais{\sCell}$ \\
  \end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigReach$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
    \begin{compactitem}
    \item $\inter{\fEpsilon}{\Ai}$ is the empty sequence
		\item $\inter{[i]}{\Ai}$ is the sequence containing $i \in
					\Ais{\sAddr}$ as the only element
		\item $\left(\left[i_1 \,..\, i_n\right], 
				\left[j_1\,..\,j_m\right],
				\left[i_1\,..\,i_n, j_1\,..\,j_m\right]\right)
					\in \inter{\pAppend}{\Ai}$ iff $i_k\neq j_l$
		\item $(m, \aInit, \aEnd, l, p) \in \inter{\pReachK}{\Ai}$
				iff $\aInit=\aEnd$ and $p = \fEpsilon$, or
				there exist addresses $a_1, \ldots, a_n \in \Ais{\sAddr}$
				such that:
		\end{compactitem}
		\hs{1.4} $\begin{array}{ll}
			\trm{(a) } p = [a_1\,..\,a_n]  \phantom{aaaa}&
			\trm{(c) } m(a_r).\inter{\fNext}{\Ai}[l]
						= a_{r+1}, \;\;\text{for}\;\;\;r < n \\
			\trm{(b) } a_1 = \aInit &
			\trm{(d) } m(a_n).\inter{\fNext}{\Ai}[l] = \aEnd
    \end{array}$ \\
  \end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigBridge$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
    \begin{compactitem}
		\item $\inter{\fPathToSet}{\Ai}(p)
					= \{ a_1, \ldots, a_n\}$ for $p
					= [a_1, \ldots, a_n] \in \Ais{\sPath}$
		\item $\inter{\fAddrToSetK}{\Ai}(m, a, l)
					= \big\{a' \in \Ais{\sAddr} | \exists p \in \Ais{\sPath}$ 
						. $(m,a,a',l,p) \in \pReachK
						\big\}$
		\item $\inter{\fGetpK}{\Ai}(m,\aInit,\aEnd,l) =
			\begin{cases}
				p & \text{if } (m,\aInit,\aEnd,l,p)
					\in \inter{\pReachK}{\Ai} \\
				\fEpsilon & \text{otherwise}
			\end{cases}$
    \end{compactitem} \\
    \hs{1} for each
      $m \in \Ais{\sMem}$,
			$p \in \Ais{\sPath}$,
			$l \in \Ais{\sLevelK}$
			and $\aInit, \aEnd \in \Ais{\sAddr}$ \\
    \begin{compactitem}
    \item $\inter{\pOrdList}{\Ai}\left(m,p \right)$
			iff
			\begin{compactitem}
				\item $p=\fEpsilon$, or
				\item $p = \lbrack a \rbrack$, or
				\item $p = [a_1\,..\, a_n]$ with $n \geq 2$ and
						$m(a_i).\inter{\key}{\Ai} \pOrd
						m(a_{i+1}).\inter{\key}{\Ai}$
						for all $1 \leq i < n$,
						for any $m \in \Ais{\sMem}$
			\end{compactitem}
		\end{compactitem} \\
  \end{tabular} \\ \\
\hline \\
\end{tabular}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSLK PATH Auxiliary functions
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\SkiplistTPathFig}{
\renewcommand{\arraystretch}{1.1}
\centering
\begin{tabular}{l}
	\hline
	$\fApp : \sSeq \times \sSeq \to \sSeq$ \\
	$\fApp (\fNil, l) = l$ \\
	$\fApp(\fCons(a,l), l') = \fCons(a, \fApp(l, l'))$ \\
	\hline
	$\fSeqToSet : \sSeq \to \sSet$ \\
	$\fSeqToSet (\fNil) = \emptyset$ \\
	$\fSeqToSet (\fCons(a,l)) = \{ a \} \cup \fSeqToSet(l)$ \\
	\hline
	$\fIsPath : \sSeq$ \\
	$\fIsPath(\fNil)$ \\
	$\fIsPath(\fCons(a, \fNil))$ \\
	$\{a\} \nsubseteq \fSeqToSet(l) \land \fIsPath(l) \Impl
		\fIsPath(\fCons(a,l))$ \\
	\hline
	$\fLast : \sSeq \to \sAddr$ \\
	$\fLast(\fCons(a, \fNil)) = a$ \\
	$l \neq \fNil \Impl \fLast(\fCons(a, l)) = \fLast(l)$ \\
	\hline
	$\pIsReachK : \sMem \times \sAddr \times \sAddr \times \sLevelK$ \\
	$\pIsReachK(m, a, a, l)$ \\
	$m[a].\fNext[l] = a' \land \pIsReachK(m, a', b, l)
		\Impl \pIsReachK(m, a, b, l)$ \\
	\hline
	$\pIsReachKP : \sMem \times \sAddr \times \sAddr \times \sLevelK
		\times \sSeq$ \\
	$\pIsReachKP(m, a, a, l, \fNil)$ \\
	$m[a].\fNext[l] = a' \land \pIsReachP(m, a', b, l, p)
		\Impl \pIsReachP(m, a, b, l, \fCons(a, p))$ \\
%	\hline
%	$\fFirstMarked : \sMem \times \sSeq \times \sLevelK \times \sAddr$ \\
%	\hline
%	$\fFirstMarked (m, \fNil, l, \fNull)$ \\
%	$p \neq \fNil \land p = \fCons(a, q)
%		\land m[a].\fLockID[l] \neq \oslash
%			\Impl \fFirstMarked(m, p, l, a)$ \\
%	$p \neq \fNil \land p = \fCons(a, q)
%		\land m[a].\fLockID[l] = \oslash
%			\land \fFirstMarked(m, q, l, b)
%				\Impl \fFirstMarked(m, p, l, b)$ \\
%	\hline
	\hline
	$\pOrdPath : \sMem \times \sSeq$ \\
	$\pOrdPath(h, \fNil)$ \\
	$h[a].\fNext[\fLevel{0}] = a' \land h[a].\fKey \pOrd h[a'].\fKey
		\land p = \fCons(a, q) \land \pOrdPath(h, q)
			\Impl \pOrdPath(h, p)$ \\
	\hline
	%\hline
	%$\pContAtLevelK : \sMem \times \sAddr \times \sAddr \times \sLevelK
		%\times \sAddr \times \sAddr \times \sLevelK \times \sSetT$ \\
	%\hline
	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$l = 0$ & \land & \center$\contained$
	%\end{array}
	%\end{pmatrix}
		%\Impl \pContAtLevelK(h, L, U, H, a, a, 0, \stSingle{t}) $ \\
	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$l = 0$ & \land & \center$\lnot \contained$
	%\end{array}
	%\end{pmatrix}
		%\Impl \pContAtLevelK(h, L, U, H, a, a, 0, \stEmpty)$ \\
	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$l > 0$ & \land & \center$\contained$
	%\end{array}
	%\end{pmatrix}
		%\land \pContAtLevelK(h,L,U,H,L,U,l-1,s)
		%\Impl \pContAtLevelK(h, L, U, H, a, a, l-1,
									%s \stCup \stSingle{t})$ \\
	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$l > 0$ & \land & \center$\lnot \contained$
	%\end{array}
	%\end{pmatrix}
		%\land \pContAtLevelK(h,L,U,H,L,U,l-1,s)
		%\Impl \pContAtLevelK(h, L, U, H, a, a, l-1, s)$ \\

	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a \neq U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$a \neq a'$ & \land & \center$\contained$ & \land \\
	%& & \center$h[a].\fNext = a'$
	%\end{array}
	%\end{pmatrix}
		%\land \pContAtLevelK(h,L,U,H,a',b,l,s)
		%\Impl \pContAtLevelK(h, L, U, H, a, b, l,s \stCup \stSingle{t})$\\
	%$\begin{pmatrix}
	%\begin{array}{p{2.5em}cp{7em}c}
	%\center$a \neq U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	%\center$a \neq a'$ & \land & \center$\lnot \contained$ & \land \\
	%& & \center$h[a].\fNext = a'$
	%\end{array}
	%\end{pmatrix}
		%\land \pContAtLevelK(h,L,U,H,a',b,l,s)
		%\Impl \pContAtLevelK(h, L, U, H, a, b, l,s)$\\
	%\hline
\end{tabular}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSLK PATH Auxiliary functions
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TSLKPathExtension}{
\renewcommand{\arraystretch}{1.1}
\centering
\begin{array}{l}
	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$l = 0$ & \land & \center$\contained$
	\end{array}
	\end{pmatrix}
		\Impl \pContAtLevelK(h, L, U, H, a, a, 0, \stSingle{t}) \\
	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$l = 0$ & \land & \center$\lnot \contained$
	\end{array}
	\end{pmatrix}
		\Impl \pContAtLevelK(h, L, U, H, a, a, 0, \stEmpty) \\
	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$l > 0$ & \land & \center$\contained$
	\end{array}
	\end{pmatrix}
		\land \pContAtLevelK(h,L,U,H,L,U,l-1,s)
		\Impl \pContAtLevelK(h, L, U, H, a, a, l-1,
									s \stCup \stSingle{t}) \\
	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a = U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$l > 0$ & \land & \center$\lnot \contained$
	\end{array}
	\end{pmatrix}
		\land \pContAtLevelK(h,L,U,H,L,U,l-1,s)
		\Impl \pContAtLevelK(h, L, U, H, a, a, l-1, s) \\

	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a \neq U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$a \neq a'$ & \land & \center$\contained$ & \land \\
	& & \center$h[a].\fNext = a'$
	\end{array}
	\end{pmatrix}
		\land \pContAtLevelK(h,L,U,H,a',b,l,s)
		\Impl \pContAtLevelK(h, L, U, H, a, b, l,s \stCup \stSingle{t}) \\
	\begin{pmatrix}
	\begin{array}{p{2.5em}cp{7em}c}
	\center$a \neq U$ & \land & \center$t=h[a].\fLockID[l]$ & \land \\
	\center$a \neq a'$ & \land & \center$\lnot \contained$ & \land \\
	& & \center$h[a].\fNext = a'$
	\end{array}
	\end{pmatrix}
		\land \pContAtLevelK(h,L,U,H,a',b,l,s)
		\Impl \pContAtLevelK(h, L, U, H, a, b, l,s)\\
\end{array}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   Translation Examples
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tslkExampleSkiplist}{
\begin{tabular}{p{14em}>{\hspace{1em}}p{24em}}

\hline
Original term & \TSLK term \\
\hline \\

\begin{array}{c}
	\pOrdList(h, sl, 0)
\end{array} &
\begin{array}{lcl}
	\overbrace{p = \fGetpK(h, \head, \fNull, 0)}^{\sigBridge} & \land &
	   \overbrace{\pOrdList(h,p)}^{\sigBridge}
\end{array} \\\\

\hline \\

\begin{array}{c}
	h[sl].\tail.\fNext[0] = \fNull \\
	\land \cdots \land \\
	h[sl].\tail.\fNext[3] = \fNull \\
\end{array} &
\begin{array}{lcccc}
	\overbrace{c_{\tail} = h[\tail]}^{\sigMemory} & \land &
		\overbrace{a_{\tail_0} = c_{\tail}.\fNext[0]}^{\sigCells} & \land&
		\overbrace{a_{\tail_0} = \fNull}^{\sigAddr} \\
	& \land & \vdots & \land & \vdots \\
	&&	\overbrace{a_{\tail_3} = c_{\tail}.\fNext[3]}^{\sigCells} & \land&
		\overbrace{a_{\tail_3} = \fNull}^{\sigAddr} \\
\end{array} \\\\

\hline

\begin{array}{ll}
	\SubList( h,& sl.\head, sl.\tail, 1, \\
				& sl.\head, sl.\tail, 0) \\
	\multicolumn{2}{c}{\land \cdots \land} \\
	\SubList(h, & sl.\head, sl.\tail, 3, \\
				& sl.\head, sl.\tail, 2) \\
\end{array} &
\begin{array}{cccc}
	\overbrace{p_{\tail_0} = \fGetpK(h, \head, \tail, 0)}^{\sigBridge}
					& \land & \cdots & \land \\
	\overbrace{p_{\tail_3} = \fGetpK(h, \head, \tail, 3)}^{\sigBridge}
					& \land \\
		\overbrace{s_{\tail_0} = \fPathToSet(p_{\tail_0})}^{\sigBridge}
					& \land & \cdots & \land \\
		\overbrace{s_{\tail_3} = \fPathToSet(p_{\tail_3})}^{\sigBridge}
					& \land \\
		\overbrace{s_{\tail_1} \subseteq s_{\tail_0}}^{\sigSets}
					& \land & \cdots & \land \\
		\overbrace{s_{\tail_3} \subseteq s_{\tail_2}}^{\sigSets}
\end{array} \\\\
\hline
\end{tabular}
}



\newcommand{\tslkExamplePreconditions}{
\begin{tabular}{p{11.5em}>{\hspace{1em}}p{26.3em}}

\hline
Original term & \TSLK term \\
\hline \\

\begin{array}{c}
	x.\fKey = \newval
\end{array} &
\begin{array}{ccc}
	\overbrace{c_x = h[x]}^{\sigMemory} & \land &
	   \overbrace{c_x.\fKey = \newval}^{\sigCells}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev.\fKey < \newval
\end{array} &
\begin{array}{cccc}
	\overbrace{c_{\prev} = h[\prev]}^{\sigMemory} & \land &
	\overbrace{c_{\prev}.\fKey = k_{\prev}}^{\sigCells} & \land \\
	\overbrace{k_{\prev} \pOrd \newval}^{\sigOrd} & \land &
	\overbrace{k_{\prev} \neq \newval}^{\sigOrd}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev.\fNext[i].\fKey > \newval
\end{array} &
\begin{array}{cccc}
	\overbrace{a_{\fNext} = c_{\prev}.\fNext[i]}^{\sigCells} & \land &
	\overbrace{c_{\fNext} = h[a_{\fNext}]}^{\sigMemory} & \land \\
	\overbrace{k_{\fNext} = c_{\fNext}.\fKey}^{\sigCells} & \land \\
	\overbrace{\newval \pOrd k_{\fNext}}^{\sigOrd} & \land &
	\overbrace{\newval \neq k_{\fNext}}^{\sigOrd}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev.\fNext[i] = x.\fNext[i]
\end{array} &
\begin{array}{ccc}
	\overbrace{a_{\fNext_x} = c_x.\fNext[i]}^{\sigCells} & \land &
	\overbrace{a_{\fNext} = a_{\fNext_x}}^{\sigAddr}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev.\fLockID[i] = j
\end{array} &
\begin{array}{ccc}
	\overbrace{t_{\prev} = c_{\prev}.\fLockID[i]}^{\sigCells} & \land &
	\overbrace{t_{\prev} = j}^{\sigThId}
\end{array} \\\\

\hline \\

\begin{array}{c}
	x.\fNext[i].\fLockID[i] = j
\end{array} &
\begin{array}{cccc}
	\overbrace{c_{\fNext_x} = h[a_{\fNext_x}]}^{\sigMemory} & \land &
	\overbrace{t_{\fNext_x} = c_{\fNext_x}.\fLockID[i]}^{\sigCells}
			& \land \\
	\overbrace{t_{\fNext_x} = j}^{\sigThId}
\end{array} \\\\

\hline \\

\begin{array}{c}
	(x,i) \notin r
\end{array} &
\begin{array}{ccccc}
	\overbrace{\empty = \mrgnEmpty}^{\sigMrgn} & \land &
	\overbrace{x_{i_{\mathit{set}}} = \mrgnSingle{x,i}}^{\sigMrgn}
			& \land &
	\overbrace{\empty = r \mrgnCap x_{i_{\mathit{set}}}}^{\sigMrgn}
\end{array} \\\\

\hline \\

\begin{array}{c}
	0 \leq i \leq 3
\end{array} &
\begin{array}{l}
	\text{We must generate four different scenarios to be} \\
	\text{combined with the conjunction of the remaining literals.}\\
	\text{These scenarios are:} \\
	\begin{array}{c>{\hspace{1em}}ccc>{\hspace{3em}}c>{\hspace{1em}}ccc}
	1. & \overbrace{0 < i}^{\sigLevelK} & \land &
		\overbrace{i < 3}^{\sigLevelK} &
	3. & \overbrace{0 = i}^{\sigLevelK} & \land &
		\overbrace{i < 3}^{\sigLevelK} \\
	2. & \overbrace{0 < i}^{\sigLevelK} & \land &
		\overbrace{i = 3}^{\sigLevelK} &
	4. & \overbrace{0 = i}^{\sigLevelK} & \land &
		\overbrace{i = 3}^{\sigLevelK} \\
	\end{array}
\end{array} \\\\

\hline
\end{tabular}
}


\newcommand{\tslkExampleTransformation}{
\begin{tabular}{p{15.5em}>{\hspace{1em}}p{22em}}

\hline
Original term & \TSLK term \\
\hline \\

\begin{array}{c}
	\AT_{43}^{[j]} \land {\AT'}_{44}^{[j]}
\end{array} &
\begin{array}{ccccccc}
	\overbrace{\AT_{j_{43}}}^{\sBool} & \land &
	\overbrace{\lnot \AT_{j_{44}}}^{\sBool} & \land &
	\overbrace{{\lnot \AT'}_{j_{43}}}^{\sBool} & \land &
	\overbrace{{\AT'}_{j_{44}}}^{\sBool}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev'.\fNext[i] = x
\end{array} &
\begin{array}{ccc}
	\overbrace{a_{\fNext_{\new}} = c_{\prev_{\new}}.\fNext[i]}^{\sigCells}
			& \land &
	\overbrace{a_{\fNext_{\new}} = x}^{\sigAddr}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev'.\fKey = \prev.\fKey
\end{array} &
\begin{array}{ccc}
	\overbrace{k_{\prev_{\new}} = c_{\prev_{\new}}.\fKey}^{\sigCells}
			& \land &
	\overbrace{k_{\prev} = k_{\prev_{\new}}}^{\sigOrd}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev'.\fData = \prev.\fData
\end{array} &
\begin{array}{cccc}
	\overbrace{e_{\prev} = c_{\prev}.\fData}^{\sigCells}
			& \land &
	\overbrace{e_{\prev_{\new}} = c_{\prev_{\new}}.\fData}^{\sigCells}
			& \land \\
	\overbrace{e_{\prev} = e_{\prev_{\new}}}^{\sigElem}
\end{array} \\\\

\hline \\

\begin{array}{c}
	\prev'.\fNext[0] = \prev.\fNext[0] \\
	\land \cdots \land \\
	\prev'.\fNext[i-1] = \prev.\fNext[i-1] \\
	\land \\
	\prev'.\fNext[i+1] = \prev.\fNext[i+1] \\
	\land \cdots \land \\
	\prev'.\fNext[3] = \prev.\fNext[3]
\end{array} &
\begin{array}{cccc}
	\overbrace{a_{\prev_0} = c_{\prev}.\fNext[0]}^{\sigCells}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{i-1}} = c_{\prev}.\fNext[i-1]}^{\sigCells}
			& \land \\
	\overbrace{a_{\prev_{i+1}} = c_{\prev}.\fNext[i+1]}^{\sigCells}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{3}} = c_{\prev}.\fNext[3]}^{\sigCells}
			& \land \\
	\overbrace{a_{\prev_{\new_0}}
				= c_{\prev_{\new}}.\fNext[0]}^{\sigCells}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{\new_{i-1}}}
				= c_{\prev_{\new}}.\fNext[i-1]}^{\sigCells}
			& \land \\
	\overbrace{a_{\prev_{\new_{i+1}}}
				= c_{\prev_{\new}}.\fNext[i+1]}^{\sigCells}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{\new_{3}}}
				= c_{\prev_{\new}}.\fNext[3]}^{\sigCells}
			& \land \\
	\overbrace{a_{\prev_{\new_0}} = a_{\prev_0}}^{\sigAddr}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{\new_{i-1}}} = a_{\prev_{i-1}}}^{\sigAddr}
			& \land \\
	\overbrace{a_{\prev_{\new_{i+1}}} = a_{\prev_{i+1}}}^{\sigAddr}
			& \land & \cdots & \land \\
	\overbrace{a_{\prev_{\new_{3}}} = a_{\prev_{3}}}^{\sigAddr}
			& \land \\
	\overbrace{h' = \fUpd(h, \prev, c_{\prev_{\new}})}^{\sigMemory}
\end{array} \\\\

\hline
\end{tabular}
}


\newcommand{\lukSignature}{
\begin{array}{lclllcll}
	\sigPair & = & \big( & \{ & \multicolumn{3}{l}{ \sPair, \sThId} & \}, 
			\\
			& & & \{ & \fPair{\_}{\_} &:& \sThId \times \sThId \to\sPair\\
			& & & \{ & & & & \} \; \big) \\ \\
	\sigSetPair & = & \big( & \{ & \multicolumn{3}{l}{\sSetPair, \sPair} & 
			\}, \\
			& & & \{ & \spEmpty & : & \sSetPair, 						\\
			& & &    & \spSingle{\_} & : & \sPair \to \sSetPair,		\\
			& & &    & \spCup & : & \sSetPair \times \sSetPair
						\to \sSetPair,									\\
			& & &    & \spCap & : & \sSetPair \times \sSetPair
						\to \sSetPair,									\\
			& & &    & \spSubst & : & \sSetPair \times \sSetPair
						\to \sSetPair							  & \},	\\

			& & & \{ & \spIn & : & \sPair \times \sSetPair				\\
			& & & 	 & \spSubset & : & \sSetPair \times \sSetPair & \}
			\; \big) \\ \\
	\sigLUK & = & \big( & \{ & \multicolumn{3}{l}{
				\sMem, \sAArray, \sLArray, \sThId, \sSetT,
				\sPair, \sSetPair} & \}, \\
			& & & \{ & \fLUKSubset & : &
				\sMem \times \sAArray \times \sAArray \times \sLArray 
					\times \sAddr \times \sAddr \times \sLevelK
					\to \sSetT \\
			& & &	 & \fInterLUK & : &
				\sMem \times \sAArray \times \sAArray \times \sLArray 
					\times \sSetT \to \sSetPair \\
			& & &	 & \fEmptyLUK & : &
				\sMem \times \sAArray \times \sAArray \times \sLArray 
					\times \sAddr \times \sAddr \times \sLevelK
					\to \sSetT \\
			& & &	 & \fMinLUK & : &
				\sMem \times \sAArray \times \sSetT \to \sThId	& \} \\
			& & & \{ & & & & \} \; \big) \\
\end{array}
}

\newcommand{\lukInterpretation}{
\begin{array}{rcl>{\hspace{-0.5em}}l>{\hspace{-0.5em}}c>{\hspace{-0.2em}}cclll}
\inter{\fLUKSubset}{\Ai}(m,L,U,H,a_1,a_2,l) & = &
		& \big\{ &
			t' & \in & \Ais{\sThId} &|&
				a_1 \leq L(t') \text{ and } U(t') \leq a_2 \text{ and } \\
		&&&&&&&&	(H(t') < l \text{ or } H(t') = l) & \big\} \\ \\

\inter{\fInterLUK}{\Ai}(m,L,U,H,g) & = &
		& \big\{ &
			\fPair{t_1}{t_2} & \in & \Ais{\sPair} &|&
				t_1 \in g \text{, } t_2 \in g \text{, } \\
		&&&&&&&&	\intersects(t_1, t_2) \text{ and } t_1 \neq t_2
		& \big\} \\ \\

\inter{\fEmptyLUK}{\Ai}(m,L,U,H,a_1,a_2,l) & = &
		& \big\{ &
			t' & \in & \Ais{\sThId} &|&
				t' \in \inter{\fLUKSubset}{\Ai}(m,L,U,H,a_1,a_2,l) \\
		&&&& \multicolumn{5}{l}{
				\text{and }
					\inter{\fLUKSubset}{\Ai}(m,L,U,H,L(t'),U(t'),H(t'))
					= \emptyset}
		& \big\} \\ \\

\inter{\fMinLUK}{\Ai}(m,U,g) & = &
		\multicolumn{8}{l}{
		\left\{\begin{array}{>{\hspace{0.3em}}l>{\hspace{2em}}l}
				\oslash & \text{if } g = \emptyset \\
				t_i & \text{if } g = \{t_1, \ldots, t_q\} \text{, }
					i \in 1..q \text{ and} \\
				& \hspace{1em} \text{forall } j \in 1..q \;
					U(t_j) \leq U(t_i)
		\end{array}\right.}
\end{array}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSL Signature - Table
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\TSLSignature}{
\centering
\begin{tabular}{r>{\vspace{-.5\baselineskip}}p{9cm}}
\hline
\textbf{Signature:} & \sigLevel \\
\textbf{Sorts:} & \sLevel \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			$0$ & : & \sLevel \\
			$s$ & : & \sLevel \to \sLevel \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			$<$  & : & \sLevel \times \sLevel \\
			\end{array} \\
\hline
%\textbf{Signature:} & \sigOrd \\
%\textbf{Sorts:} & \sOrd \\
%\textbf{Functions:} &
%			\begin{array}{p{2cm}cl}
%				\fZero & : & \sOrd \\
%				\fInfty & : & \sOrd \\
%			\end{array} \\
%\textbf{Predicates:} &
%			\begin{array}{p{2cm}cl}
%			\pOrd	& : & \sOrd \times \sOrd \\
%			\end{array} \\
%\hline
\textbf{Signature:} & \sigArray \\
\textbf{Sorts:} & \sArray, \sLevel, \sAddr \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fArrayRd{\_}{\_} &:& \sArray \times \sLevel \to \sAddr \\
			\fArrayUpd{\_}{\_}{\_} & : &
				\sArray \times \sLevel \times \sAddr \to \sArray \\
			\end{array} \\
\hline
\textbf{Signature:} & \sigCells \\
\textbf{Sorts:} & \sCell, \sElem, \sOrd, \sArray, \sAddr, \sLevel \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fError & : & \sCell \\
			\fMkcell & : & \sElem \times \sOrd \times \sArray \times \sLevel
												\to \sCell \\
			$\_.\fData$ & : & \sCell \to \sElem \\
			$\_.\fKey$ & : & \sCell \to \sOrd \\
			$\_.\fArr$ & : & \sCell \to \sArray \\
			$\_.\fMax$ & : & \sCell \to \sLevel \\
			\end{array} \\
\hline
%\textbf{Signature:} & \sigMemory \\
%\textbf{Sorts:} & \sMem, \sAddr, \sCell \\
%\textbf{Functions:} &
%			\begin{array}{p{2cm}cl}
%			\fNull & : & \sAddr \\
%			\fRd & : & \sMem \times \sAddr \to \sCell \\
%			\fUpd & : & \sMem \times \sAddr \times \sCell \to \sMem
%			\end{array} \\
%\hline
\textbf{Signature:} & \sigReach \\
\textbf{Sorts:} & \sMem, \sAddr, \sPath \\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fEpsilon & : & \sPath \\
			\lbrack \_ \rbrack & : & \sAddr \to \sPath
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pAppend & : & \sPath \times \sPath \times \sPath \\
			\pReach & : & \sMem \times \sAddr \times \sAddr \times \sLevel
											\times \sPath \\
			\end{array} \\
\hline
%\textbf{Signature:} & \sigSets \\
%\textbf{Sorts:} & \sAddr, \sSet \\
%\textbf{Functions:} &
%			\begin{array}{p{2cm}cl}
%			$\emptyset$ & : & \sSet \\
%			$\{ \_ \}$ & : & \sAddr \to \sSet \\
%			$\cup$, $\cap$, $\setminus$ & : & \sSet \times \sSet \to \sSet
%			\end{array} \\
%\textbf{Predicates:} &
%			\begin{array}{p{2cm}cl}
%			\pAppend & : & \sPath \times \sPath \times \sPath \\
%			\pReach & : & \sMem \times \sAddr \times \sAddr \times \sLevel
%											\times \sPath \\
%			\end{array} \\
%\hline
\textbf{Signature:} & \sigBridge \\
\textbf{Sorts:} & \sMem, \sAddr, \sSet, \sPath, \sLevel\\
\textbf{Functions:} &
			\begin{array}{p{2cm}cl}
			\fPathToSet & : & \sPath \to \sSet \\
			\fAddrToSet & : & \sMem \times \sAddr \times \sLevel
				\to \sSet \\
			\fGetp & : & \sMem \times \sAddr \times \sAddr \times
				\sLevel \to \sPath \\
			\end{array} \\
\textbf{Predicates:} &
			\begin{array}{p{2cm}cl}
			\pOrdList & : & \sMem \times \sPath \\
			\pSkiplist & : & \sMem \times \sSet \times \sLevel \times \sAddr
												\times \sAddr \\
			\end{array} \\
\hline
\end{tabular}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   TSL Interpretations
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\TSLInterpretations}{
\centering
\begin{tabular}{p{11cm}}
\hline \\
\textbf{Signature:} $\sigLevel$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
		\begin{compactitem}
			\item $\inter{0}{\Ai} = 0$
			\item $\inter{s}{\Ai}(l) = s(l)$
		\end{compactitem} \\
		for each
			$l \in \Ais{\sLevel}$ \\
	\end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigArray$ \\
\textbf{Interpretations:} \\
  \hspace{1.5em}
  \begin{tabular}{p{10cm}}
		\begin{compactitem}
			\item $\fArrayRdInter{A}{l}{\Ai} = A(l)$
			\item $\fArrayUpdInter{A}{l}{a}{\Ai} = A_{\mathit{new}}$, where
				$A_{\mathit{new}}(l) = a$ and
				$A_{\mathit{new}}(i) = A(i)$ for $i \neq l$
		\end{compactitem} \\
		for each
			$A, A_{\mathit{new}} \in \Ais{\sArray}$,
			$l \in \Ais{\sLevel}$ and
			$a \in \Ais{\sAddr}$ \\
	\end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigCells$ \\
\textbf{Interpretations:} \\
	\hspace{1.5em}
  \begin{tabular}{p{10cm}}
		\begin{compactitem}
		\item $\inter{\fMkcell}{\Ai} (e, k, \vect{a}, l) =
						\langle e, k, A, l \rangle$
		\item $\inter{\fError}{\Ai}.\inter{\fArr}{\Ai}(l) = \inter{\fNull}{\Ai}$
		\item $\langle e, k, A, l \rangle.\inter{\fData}{\Ai} = e$
		\item $\langle e, k, A, l \rangle.\inter{\fKey}{\Ai} = k$
		\item $\langle e, k, A, l \rangle.\inter{\fArr}{\Ai} = A$
		\item $\langle e, k, A, l \rangle.\inter{\fMax}{\Ai} = l$
		\end{compactitem} \\
		for each
			$e \in \Ais{\sElem}$,
			$k \in \Ais{\sOrd}$,
			$A \in \Ais{\sArray}$,
			and $l \in \Ais{\sLevel}$ \\
	\end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigReach$ \\
\textbf{Interpretations:} \\
	\hspace{1.5em}
  \begin{tabular}{p{10cm}}
		\begin{compactitem}
		\item $(m, \aInit, \aEnd, l, p) \in \inter{\pReach}{\Ai}$
			iff $\aInit=\aEnd$ and $p = \fEpsilon$, or
		there exist addresses $a_1, \ldots, a_n \in \Ais{\sAddr}$ such 
		that:
		\end{compactitem} \\
		\hs{1.4} $\begin{array}{ll}
			\trm{(a) } p = [a_1\,..\,a_n]  \phantom{aaaa}&
			\trm{(c) } m(a_r).\inter{\fArr}{\Ai}(l)
				= a_{r+1}, \;\;\;\text{for}\;\;\;r < n \\
			\trm{(b) } a_1 = \aInit &
			\trm{(d) } m(a_n).\inter{\fArr}{\Ai}(l)
				= \aEnd
		\end{array}$ \\
	\end{tabular} \\ \\
\hline \\
\textbf{Signature:} $\sigBridge$ \\
\textbf{Interpretations:} \\
	\hspace{1.5em}
	\begin{tabular}{p{10cm}}
		\begin{compactitem}
		\item $\inter{\fAddrToSet}{\Ai}(m, a, l)
					= \big\{a' \in \Ais{\sAddr} | \exists p \in \Ais{\sPath}$ .  
						$(m,a,a',l,p) \in \pReach
						\big\}$
		\item $\inter{\fGetp}{\Ai}(m,a_i,a_e,l) =
			\begin{cases}
				p & \text{if } (m,a_i,a_e,l,p)
					\in \inter{\pReach}{\Ai} \\
				\fEpsilon & \text{otherwise}
			\end{cases}$
		\item $\inter{\pSkiplist}{\Ai}(m, r, l, a_i, a_e)$ iff
				$\begin{bmatrix}
					\begin{array}{cl}
						\inter{\pOrdList}{\Ai}(m, \inter{\fGetp}{\Ai}(m, a_i, a_e, 0))
								& \land \\
						r = \inter{\fPathToSet}{\Ai}(\inter{\fGetp}{\Ai}(m,a_i,a_e,l)) & \land \\
						0 \leq l \land
						\forall a \in r \;.\;
							m(a).\inter{\fMax}{\Ai} \leq l & \land \\
						m(a_e).\inter{\fArr}{\Ai}(l) = \inter{\fNull}{\Ai}
							& \land \\
						\big( 0 = l_{\fMax} \big) \; \lor \\
							\big(\exists l_p \;.\; \inter{s}{\Ai}(l_p) = l \land
								\;\forall\; i \in 0, \ldots, l_p \;.\; \\
								\hspace{1em} m(a_e).\inter{\fArr}{\Ai}(i)
									= \inter{\fNull}{\Ai} \; \land \\
								\hspace{1em}
									\inter{\fPathToSet}{\Ai}(
										\inter{\fGetp}{\Ai}(m, a_i, a_e,
											\inter{s}{\Ai}(i))) \subseteq \\
								\hspace{2em} \inter{\fPathToSet}{\Ai}(
										\inter{\fGetp}{\Ai}(m, a_i, a_e, i)) \big)
					\end{array}
				\end{bmatrix}$
		\end{compactitem} \\
		for each
      $m \in \Ais{\sMem}$,
			$p \in \Ais{\sPath}$,
			$r \in \Ais{\sSet}$,
			$l \in \Ais{\sLevelK}$
			and $a, a_i, a_e \in \Ais{\sAddr}$ \\
	\end{tabular} \\ \\
\hline \\

\end{tabular}
}


